KinScene: Model-Based Mobile Manipulation of Articulated Scenes

Sequentially interacting with articulated objects is crucial for a mobile manipulator to operate effectively in everyday environments. To enable long-horizon tasks involving articulated objects, this study explores building scene-level articulation models for indoor scenes through autonomous exploration. While previous research has studied mobile manipulation with articulated objects by considering object kinematic constraints, it primarily focuses on individual-object scenarios and lacks extension to a scene-level context for task-level planning. To manipulate multiple object parts sequentially, the robot needs to reason about the resultant motion of each part and anticipate its impact on future actions. We introduce KinScene, a full-stack approach for long-horizon manipulation tasks with articulated objects. The robot maps the scene, detects and physically interacts with articulated objects, collects observations, and infers the articulation properties. For sequential tasks, the robot plans a feasible series of object interactions based on the inferred articulation model. We demonstrate that our approach repeatably constructs accurate scene-level kinematic and geometric models, enabling long-horizon mobile manipulation in a real-world scene. Code and additional results are available at https://chengchunhsu.github.io/KinScene/

==> backup/_2._related.tex <==
\section{Related Work}
In this section, we delve into previous research efforts related to the subproblems associated with scene-level articulation object manipulation.

% In this section we discuss prior effort on the sub problem
% note that they explore the problem separately rather than a whole

% ~\todo{finish this}

% \subsection{Scene Mapping}
% limit to static model
% we are first to propose full-stack approach for articulation mapping


\noindent \textbf{Articulation Model Estimation.}
% limited to tabletop environment
% category-dependent
% input: occlusion / view angle
% our approach is agnostic to articulation estimatoin
% we study the effectiveness of different methods in unstructured indoor environments
Articulation model estimation methods infer the object parts and kinematic constraints between them. Previous approaches utilized probabilistic methods~\cite{dearden2005learning, sturm2008adaptive, sturm2008unsupervised, sturm2009learning} to infer these constraints through part tracking. However, their practical applicability in natural environments is limited due to the requirement of markers and handcrafted features. Leveraging large-scale 3D datasets~\cite{wang2019shape2motion, mao2022multiscan}, recent methods have employed learning-based approaches for articulation estimation from raw sensory input including images~\cite{zeng2021visual}, videos~\cite{qian2022understanding}, and point clouds~\cite{li2020category, wang2019shape2motion, weng2021captra, noguchi2021neural, hameed2022learning}. These models exhibit limited generalization to arbitrary unseen objects as they heavily rely on category-level priors for articulation parameter estimation. Recent studies have proposed category-independent methods~\cite{jain2020screwnet, jiang2022opd, sun2023opdmulti, heppert2022category, jiang2022ditto} to alleviate dependence on object categories. 
% Articulation models represent the object parts and the kinematics (and sometimes dynamics) relationships between them. Earlier works model the object partonomy and articulation with probabilistic methods~\cite{dearden2005learning,sturm2008adaptive,sturm2008unsupervised,sturm2009learning}. They typically rely on markers or handcrafted features to track the mobile parts, limiting their practical applicability in natural environments. In recent years, deep learning methods~\cite{omran2018neural,li2020category,wang2019shape2motion,weng2021captra,noguchi2021neural,hameed2022learning} have been employed for articulation estimation from raw sensory data. The majority of these works predict articulation models from single observations. They rely on category-level prior to estimating articulation parameters. For this reason, they are category-dependent and cannot generalize to diverse daily objects in indoor scenes. 

\noindent \textbf{Articulated Object Manipulation.}
Manipulating articulated objects has been a persistent challenge in robotics. This involves coordinating the robot's movements to ensure that the action sequence aligns with the kinematic constraints of the objects. 

Previous approaches suggested inferring motion trajectories from single initial observation~\cite{xu2022universal}, yet a single initial observation remains inherently ambiguous as it does not reveal the underlying kinematic joints.
%
Additionally, some work suggests inferring the affordance and applied action based on initial or per-step observations without explicitly modeling the articulation parameters~\cite{mo2021where2act, eisner2022flowbot3d, zhang2023flowbot++}. However, since these actions need to be estimated at each time step, they lack the capability for long-horizon planning.

Another line of work suggested explicitly estimating articulation parameters through exploratory actions~\cite{wherewang2022adaafford, nie2023structure, wu2024learning}
to facilitate sophisticated planning and manipulation. These actions can be created by scripted action~\cite{jiang2022ditto} or learned policies~\cite{kumar2019estimating, gadre2021act, lv2022sagci}. However, these studies are limited to controlled laboratory settings, primarily focusing on modeling a singulated object in a tabletop environment. Therefore, they lack the ability for interaction in a real-world indoor environment with life-size articulated objects.



articulation parameters from interactions to guide downstream manipulation tasks~\cite{}

these methods deduce the interaction hotspot and applied action based on observations at each step. However, these studies are limited to controlled laboratory settings, primarily focusing on modeling a singulated object in a tabletop environment. Therefore, they lack the ability for long-horizon planning and interaction in a real-world indoor environment with life-size articulated objects.

learns to predict per-point motion of articulated objects under instantaneous motion. While the per-point motion affordance learning of \cite{eisner2022flowbot3d} outperforms previous approaches, it does not explicitly model the articulation parameters. Thus, the affordance needs to be estimated in each time step,


~\cite{nie2022structure} proposed a similar idea of estimating articulation parameters from interactions to guide downstream manipulation tasks. However, our method does not require \textit{a priori} interactions with the manipulated objects.

% limitation of zero-shot approach - cannot plan because of single-step action
In contrast, another line of research involves interacting with articulated objects through exploration~\cite{}. Specifically, these methods deduce the interaction hotspot and applied action based on observations at each step. However, these studies are limited to controlled laboratory settings, primarily focusing on modeling a singulated object in a tabletop environment. Therefore, they lack the ability for long-horizon planning and interaction in a real-world indoor environment with life-size articulated objects.



These studies are constrained to controlled laboratory settings, primarily focusing on modeling individual objects in tabletop environments, thereby limiting their applicability to broader indoor environments.

% manipulation - does not lead to fully-fledge articulation model
% interactive perception - scripted actions?

% limitation of zero-shot approach - unreliable because of lack of exploration
Previous approaches suggested estimating articulation parameters from a single view to facilitate sophisticated planning and manipulation~\cite{}. However, articulation estimation from a single initial observation remains inherently ambiguous. Mobile parts may either move along a prismatic axis or rotate around a revolute axis, depending on the underlying kinematic joints.
% limitation of zero-shot approach - cannot plan because of single-step action
In contrast, another line of research involves interacting with articulated objects through exploration~\cite{}. Specifically, these methods deduce the interaction hotspot and applied action based on observations at each step. However, these studies are limited to controlled laboratory settings, primarily focusing on modeling a singulated object in a tabletop environment. Therefore, they lack the ability for long-horizon planning and interaction in a real-world indoor environment with life-size articulated objects.


Recent research has employed physical interaction to generate informative motion through either scripted actions~\cite{jiang2022ditto} or learned policies~\cite{kumar2019estimating, gadre2021act, lv2022sagci}. Based on changes in object state, these studies infer the articulation model by incorporating hierarchical recursive Bayesian filters~\cite{martin2016integrated}, probabilistic models~\cite{sturm2011probabilistic}, feature tracking~\cite{pillai2015learning}, or geometric deep learning techniques~\cite{}.

lack of self-exploration ability
infer none or incomplete articulation model


The most closely related work~\cite{hsu2023ditto} aims to construct the articulation model of an indoor environment through a robot's self-directed exploration but is primarily focused on building digital twins without real-world evaluation. Additionally, it simplifies physical exploration in simulation and lacks direct transferability to real mobile manipulators.



% . Based on changes in object state, these studies infer the articulation model by incorporating hierarchical recursive Bayesian filters~\cite{martin2016integrated}, probabilistic models~\cite{sturm2011probabilistic}, and feature tracking~\cite{pillai2015learning}.


% Katz et al.\cite{katz2013interactive} pioneered interactive perception\cite{bohg2017interactive} for articulation model estimation. Subsequent studies expanded on this by incorporating hierarchical recursive Bayesian filters~\cite{martin2016integrated}, probabilistic models~\cite{sturm2011probabilistic}, and feature tracking~\cite{pillai2015learning}. Recent advancements in this area leverage informative motion generated through either handcrafted strategies~\cite{jiang2022ditto} or learned policies~\cite{kumar2019estimating, gadre2021act, lv2022sagci}, estimating articulation models using geometric deep learning techniques. However, these methods are tailored for individual objects and face challenges when applied to large indoor environments with multiple objects at unknown locations. 


% Previous studies leverage physical interaction to create informative motion and infer the articulation model based on object state changes. Katz \etal~\cite{katz2013interactive} is the pioneer work that introduces interactive perception~\cite{bohg2017interactive} for articulation model estimation. Some following works extend it with hierarchical recursive Bayesian filters~\cite{martin2016integrated}, probabilistic models~\cite{sturm2011probabilistic}, and feature tracking~\cite{pillai2015learning}. Recent work in this direction utilizes the informative motion created by handcrafted strategies~\cite{jiang2022ditto} or learned policy~\cite{kumar2019estimating,gadre2021act,lv2022sagci} and estimate articulation models with geometric deep learning techniques. The methods above are designed for individual objects. They cannot be easily extended to large indoor environments with multiple objects at unknown locations. The closest work~\cite{hsu2023ditto} aims to build the articulation model of an indoor environment through a robot’s self-directed exploration, yet it focuses solely on building digital twins without real-world evaluation. Plus, it simplifies the physical exploration in simulation and is not directly transferable in real mobile manipulators. 


% Specifically, these methods deduce the interaction hotspot and applied action based on observations at each step. However, these studies are limited to controlled laboratory settings, primarily focusing on modeling a singulated object in a tabletop environment. Therefore, they lack the ability for long-horizon planning and interaction in a real-world indoor environment with life-size articulated objects.


% Physical exploration create 
% Previous studies leverage physical interaction to create novel sensory stimuli and infer the articulation model based on object state changes. Katz \etal~\cite{katz2013interactive} is the pioneer work that introduces interactive perception~\cite{bohg2017interactive} for articulation model estimation. Some following works extend it with hierarchical recursive Bayesian filters~\cite{martin2016integrated}, probabilistic models~\cite{sturm2011probabilistic}, and feature tracking~\cite{pillai2015learning}. Recent work in this direction utilizes the informative motion created by handcrafted strategies~\cite{jiang2022ditto} or learned policy~\cite{kumar2019estimating,gadre2021act,lv2022sagci} and estimate articulation models with geometric deep learning techniques. The methods above are designed for individual objects. They cannot be easily extended to large indoor environments with multiple objects at unknown locations. The closest work~\cite{hsu2023ditto} aims to build the articulation model of an indoor environment through a robot’s self-directed exploration, yet it focuses solely on building digital twins without real-world evaluation. Plus, it simplifies the physical exploration in simulation and is not directly transferable in real mobile manipulators. 




% Another line of work leverages physical interaction to create novel sensory stimuli and infer the articulation model based on object state changes. Katz \etal~\cite{katz2013interactive} is the pioneer work that introduces interactive perception~\cite{bohg2017interactive} for articulation model estimation. Some following works extend it with hierarchical recursive Bayesian filters~\cite{martin2016integrated}, probabilistic models~\cite{sturm2011probabilistic}, and feature tracking~\cite{pillai2015learning}. Recent work in this direction utilizes the informative motion created by handcrafted strategies~\cite{jiang2022ditto} or learned policy~\cite{kumar2019estimating,gadre2021act,lv2022sagci} and estimate articulation models with geometric deep learning techniques. The methods above are designed for individual objects. They cannot be easily extended to large indoor environments with multiple objects at unknown locations. In contrast, our approach develops a category-independent approach that actively explores the environment and builds scene-level articulation models.

% % limitation of zero-shot approach - unreliable because of lack of exploration
% Manipulating articulated objects has been a persistent challenge in robotics. This involves coordinating the robot's base and arm movements to ensure that the action sequence aligns with the kinematic constraints of the objects. Previous approaches suggested estimating articulation parameters from a single view to facilitate sophisticated planning and manipulation~\cite{}. However, articulation estimation from a single initial observation remains inherently ambiguous. Mobile parts may either move along a prismatic axis or rotate around a revolute axis, depending on the underlying kinematic joints.
% % limitation of zero-shot approach - cannot plan because of single-step action
% In contrast, another line of research involves interacting with articulated objects through exploration~\cite{}. Specifically, these methods deduce the interaction hotspot and applied action based on observations at each step. However, these studies are limited to controlled laboratory settings, primarily focusing on modeling a singulated object in a tabletop environment. Therefore, they lack the ability for long-horizon planning and interaction in a real-world indoor environment with life-size articulated objects.


% \subsection{Articulation Planning and Manipulation}



% \subsection{Articulation Manipulation and Planning}
% exploration
% single step action
% limited to tabletop environment

% discuss the planning paper: Predicting Motion Plans for Articulating Everyday Objects
% check Ben's note

% we study task-level long-horizon planning

% \subsection{Full-stack attempt(?)}

==> backup/_3._formulation.tex <==
\section{Problem Formulation}
\label{sec: formulation}
Our overarching objective is to facilitate scene-level tasks like unloading a dishwasher or transferring raw chicken from the fridge to the oven. However, our current focus is directed at addressing the challenge of coordinating the interdependent actions of degrees of freedom essential for executing these tasks. Essentially, these tasks involve the actuation of several articulated objects in the scene in a specific sequence, requiring scene-level reasoning to determine the correct order. Hence, our problem definition centers on attaining a desired joint configuration for the articulated objects within the scene.

We posit that the articulation structure at the scene level can be effectively modeled using a~\textit{kinematic tree}. The scene is comprised of static and mobile parts. The static parts, such as the cabinet's body and the floor, are rigidly connected and immovable, forming a cohesive unit~\ie, the base model. The mobile parts are linked to the base model through kinematic constraints. To represent this configuration as a kinematic tree, the base model serves as the root, and each mobile part functions as a leaf connected to the root. The edges within the tree describe the kinematic joints between these parts. Following prior work~\cite{hsu2023ditto}, we assume each part is connected to the static base model and has only one degree of freedom.

\noindent \textbf{Scene-level Articulation Model.}
% \todo{find a way to define mobile part}
The kinematic tree $M = \langle B, V, E \rangle$ represents an indoor scene populated with articulated objects. In this representation, the root $B$ defines the geometry of the static base model, the nodes $V$ define the geometry of individual parts, and the edges $E$ define the kinematic joints between the parts. We parameterize kinematic joints following ANCSH~\cite{li2020category}. Revolute joint parameters are the direction of the revolute axis $u^r \in \mathbb{R}^{3}$ and a pivot point $q \in \mathbb{R}^{3}$ on the revolute axis. Prismatic joint parameters are the direction of the translation axis $u^p \in \mathbb{R}^{3}$. Henceforth, we will refer to this kinematic tree as a scene-level articulation model. 

\noindent \textbf{State Space.}
The state is defined by a group of rigid bodies and their respective kinematic trees. In this context, robots and articulated objects are represented as a tree interconnected through joints, which determine their degrees of freedom. Given a scene with a set of articulated objects that can be represented by $M$, we can define a state space $S=S_V \times S_R$, where $S_V$ is the state for each part in $V$ and $S_R$ is the state of the robot. The state $S_R = S_{base} \times S_{arm} \times S_{gripper}$ is defined by base pose $S_{base} \in SE(2)$ and arm pose $S_{arm} \in SE(3)$ and openness of the gripper $S_{gripper}\in \{0, 1\}$.
% The action space $A = A_{base} \times A_{arm} \times A_{gripper}$ is defined by base action $A_{base} \in SE(2)$ and arm action $A_{arm} \in SE(3)$ and openness of the gripper $A_{gripper}\in \{0, 1\}$.
% The robot's state $S_R = T_{base} \times T_{arm}$ is defined by the base pose $T_{base} \in SE(2)$ and the arm pose $T_{arm} \in SO(3)$.

\noindent \textbf{Task Definitions.}
Our focus is to achieve a desired joint configuration for the articulated objects within the scene. The robot needs to discern the correct sequence for actuating multiple articulated objects within the scene.
% The \todo{XX} task $\langle S, A, s_0, G \rangle$ can be specified by a set of goal states $G \subseteq S$. 
Given a state space $S$ and action space $A$, the task can be specified by a set of goal states $G \subseteq S$. The goal state $G$ can be specified by $(X, \Theta)$, where $X \subseteq V$, and $\Theta$ is the threshold for the goal state of each part within the set $X$. The robot must infer a plan $p\in P$ that can be represented as $p = \langle s_0,a_0,s_1,a_1,...,s_i,a_i \rangle$, where $a_0,a_1,...,a_i \in A$, $s_0,s_1,...,s_i \in S$, $s_i \in G$ and $P$ is the set of satisfactory plans.

\noindent \textbf{Solution Definitions.}
To solve the task, the robot must perform one or more object interactions to change the scene from the current to the desired configuration. We propose to formulate this task as a hierarchical planning problem.
The robot first splits the task into individual sub-goal $\langle x, \theta \rangle$, where the robots need to articulate object part $x$ until achieve goal state $\theta$. Subsequently, the robot plans the sequence of sub-goals $\pi = \langle x_0, \theta_0 \rangle, \langle x_1, \theta_1 \rangle, ..., \langle x_n, \theta_n \rangle$, where $n$ is the size of $X$. \todo{collision constraints with previous goal} Given a sub-goal $\langle x, \theta \rangle$, the robot infers a set of collision-free action trajectories $\tau_{x} = \langle s^x_0,a^x_0,s^x_1,a^x_1,...,s^x_j,a^x_j \rangle$ to articulate object part $x$.
% The robot first determines the order of manipulating parts $X = \langle x_0,x_1,...,x_n \rangle$, where $x_0,x_1,...,x_n \in v$. 
% For each object $x \in v$, the robot infers a set of collision-free action trajectories $\tau_{x} = \langle s^x_0,a^x_0,s^x_1,a^x_1,...,s^x_i,a^x_i \rangle$.
The final solution for the task is $\hat{p} = \{ \tau_{x} \} \forall x \in v$.

To infer the solution plan $\hat{p}$, we propose to find a high-level planner $f$ so that $\pi = h(G, M, s)$, and a trajectory planner $h$ so that $\tau = h(G, M, s, o)$, where $s \in S$ is the current state and $o$ is the robot's current egocentric observation. In the unboxing setting, $M$ is unavailable at the beginning. We approach the task by reconstructing the scene-level articulation model $M$ from the robot's egocentric observation by using an exploration planner $h'$ so that $\langle \tau, M \rangle = h'(G, s, o)$.

% % where $s_{i}, G \in S$. I

% % a set of parameterized actions
% % A, an initial state s0 ∈ S and a set of goal states S∗ ⊆ S

% OxA'xMxS' -> S, A

% % The \todo{XX} task can be specified by $(s_{init}, v, s_{goal})$, where $s_{init}$ is the initial state, $v$ is the subset of parts drawn from the set $V$, and $g$ is the goal joint states for each part within the set $v$.


% % To solve the task, we propose to formulate the ~\todo{XX} task as a hierarchical planning problem. For task-level planning, the robot must infer a plan by determining the order of manipulating parts within the set $v$. We define this order by $P_{task} = \langle u_0,u_1,...,u_n \rangle$, where $u_0,u_1,...,u_n \in v$ and $n$ is the size of the set $v$. For motion-level planning, the robot must infer a sequence of plan $P_{motion}$ 


% We approach the \todo{XX} task by reconstructing the scene-level articulation model $M$ from the robot's egocentric observation and self-directed exploration.


% % We formulate the ~\todo{XX} task as a hierarchical planning problem
% % To reconstruct the scene-level articulation model $M$, 


% an articulated object constitutes a kinematic tree, where the nodes define the geometry and physical properties (e.g. mass and friction) of individual parts and the edges define the kinematic joints between the parts.

% we represent the indoor scenario populated with articulation objects, where every rigid part can be represented as a flat kinematic tree




% problem:
% given a scene kinematic tree
% M = {B, [<geometry, kinematic constraints, current state>, <>, <>, ...]}
% base map, {mobile part geometry current state}, {kinematic constraints}

% task
% open {a b c} (objects) to certain degree threshold {ta tb tc}

% solution
% task-level
% order {a->b->c} degree {da, db, dc}
% motion-level
% sequence of action f(s, a) to reach goal state
% si+1 = f(ai, si) and ai ∈ A(si) for i = 0, . . . , n and sn+1 ∈ SG

% to infer action sequence, we learn the transition functions
% OxA -> S, M
% OxA -> S


% We investigate the challenge of constructing an articulation model for an indoor scene populated with articulated objects. These models play a crucial role in facilitating long-term and repeatable interactions. Articulated objects, composed of multiple parts, are defined by joints that constrain the relative motion between each pair of components. In this study, our goal is to enable the robot to segment these parts, infer an accurate articulation model, and follow the action trajectory for effective manipulation.

% % \noindent \textbf{Articulation Model.}
% The articulation model represents the kinematic constraints between object parts. We parametrize articulation following ANCSH~\cite{li2020category}. Revolute joint parameters are the direction of the revolute axis $u^r \in \mathbb{R}^{3}$, a pivot point $q \in \mathbb{R}^{3}$ on the revolute axis. Prismatic joint parameters are the direction of the translation axis $u^p \in \mathbb{R}^{3}$.

% ~\todo{mention challenge full stack, e.g., exploration}

==> backup/__intro.tex <==

Based on the static models acquired from SLAM or other 3D reconstruction techniques, the robot discovers and physically interacts with articulated objects in the environment. After that, the robot captures the change in the object's state before and after the interaction and infers the articulation properties. 



real-world situations where regions can be partially occupied, doors can be half open, and multiple doors need to be opened to enable reachability. Real-world manipulation would require a robot to depart from reconstructing a static map to unraveling the physical properties of objects.


In an unfamiliar environment, the mobile robots


These maps facilitate mobile robots for obstacle avoidance and long-horizon planning.


exploring, reconstructing, and planning in an unfamiliar environment has been an effective paradigm for mobile robots. Recent advances in structure sensors and SLAM algorithms~\cite{newcombe2011kinectfusion,newcombe2015dynamicfusion,geiger2011stereoscan} have offered ways to build a map of the environment. These maps facilitate mobile robots for obstacle avoidance and long-horizon planning.


. Nevertheless, static 3D models cannot fully represent real-world situations where regions can be partially occupied, doors can be half open, and multiple doors need to be opened to enable reachability. Real-world manipulation would require a robot to depart from reconstructing a static map to unraveling the physical properties of objects.




% How does the scene-level AE model help - and current limitations
Another line of studies uses a two-stage solution~\cite{}. For each unfamiliar object, the robot first estimates the articulation model of the objects.
These models describe the kinematic constraints, such as the position or orientation of the joint axis, of the articulation objects. By unraveling these physical properties of the object, the robot can plan for the whole action trajectory before the execution. However, articulation estimation from a single initial observation is inherently ambiguous. The mobile parts may move along a prismatic axis or rotate around a revolute axis depending on the underlying kinematic joints.
% Our strategy - exploration + exploitation
% Recent studies in interactive perception~\cite{} leverage robot's physical interactions to produce visual observations of articulated motions from which they estimate the articulation properties. 


Zero-shot manipulation systems for articulated objects have been studied. 

% limitation of zero-shot approach - cannot plan 
These studies~\cite{} infer an interaction point and action based on the observation at each timestamp as the policy for manipulation. These studies are restricted to controlled laboratory settings focused primarily on tabletop manipulation. They lack the ability for long-horizon planning since they select only the single-step action.








% limitation of static map
Jointly exploring and reconstructing an unfamiliar environment has been a paradigm for mobile robots. Recent advances in structure sensors and SLAM algorithms~\cite{newcombe2011kinectfusion,newcombe2015dynamicfusion,geiger2011stereoscan} have offered ways to build a map of the environment. These maps facilitate mobile robots for long-horizon planning and obstacle avoidance. Nevertheless, static 3D models cannot fully represent real-world situations where regions can be partially occupied, doors can be half open, and multiple doors need to be opened to enable reachability. Real-world manipulation would require a robot to depart from reconstructing a static map to unraveling the physical properties of objects.







In this work, we propose a two-stage solution, where the robots automatically build articulated models of indoor scenes from their purposeful interactions. We show that the articulated models enable zero-shot articulation planners and long-term repeatable interaction with articulation objects.

% previous studies on Component #1: build static map
Interacting with articulation objects is crucial for the robot to operate in everyday environments. Recent advances in structure sensors and SLAM algorithms~\cite{newcombe2011kinectfusion,newcombe2015dynamicfusion,geiger2011stereoscan} have offered ways to build a map of the environment. These maps facilitate mobile robots to localize themselves, navigate around, and plan for the next actions. Nevertheless, real-world manipulation would require a robot to depart from reconstructing a static scene to unraveling the physical properties of objects. To physically interact with articulation objects, such as cabinets and doors, the robot needs to understand their kinematics and articulation properties. From a task planning perspective, static 3D models cannot fully represent real-world situations where regions can be partially occupied, doors can be half open, and multiple doors need to be opened to enable reachability. Similar to how mapping guides navigation, the articulation model allows the robot to plan its actions for object manipulation. Motivated by this goal, this work aims to enable robots to automatically build articulated models of indoor scenes from their purposeful interactions. These models enable zero-shot articulation planners and long-term repeatable interaction with articulation objects.

% previous studies on Component #2: build articulation model
% with AE: static / category-dependent (/ IP)
% without AE: exploration based
Interacting with articulation objects has been a long-standing challenge in robotics. Previous work has proposed to learn the articulation parameters to enable robotic systems to successfully perform sophisticated planning and control over 3D articulated objects. A series of data-driven approaches have attempted to infer articulation from static visual observations by training models on large 3D datasets~\cite{li2020category,weng2021captra}. These models rely on category-level priors and suffer from appearance ambiguity, limiting their generalizations to a handful of preset categories. Another line of research uses online perception~\cite{} to infer a sequential interaction policy that reveals the object’s hidden part geometry and kinematics. These works primarily focus on individual objects, whereas scaling to room-sized environments requires the robot to efficiently and effectively explore the large-scale 3D space for meaningful interactions. Without the explicit modeling of articulation, these methods cannot either do long-horizon planning or guarantee long-term repeatable interactions given different base positions or view angles. The closest work~\cite{hsu2023ditto} aims to build the articulation model of an indoor environment through a robot’s self-directed exploration, yet it focuses solely on building digital twins without real-world evaluation. Plus, it simplifies the physical exploration in simulation and is not directly transferable in real mobile manipulators. 

% How do existing work get AE models? Why is it not enough for scene-level challenges?
% Understanding object articulation has been a long-standing challenge in computer vision and robotics. In recent years, a series of data-driven approaches have attempted to infer articulation from static visual observations by training models on large 3D datasets~\cite{li2020category,weng2021captra}. These models rely on category-level priors, limiting their generalizations to a handful of preset categories. Category-agnostic approach~\cite{} uses the single image of the object in its initial state, suffering from the ambiguity of articulation despite the similar object appearance. Another line of research~\cite{hausman2015active,martin2014online} uses interactive perception~\cite{bohg2017interactive}. They leverage physical interaction to emit visual observations of articulated motions from which they estimate the articulation properties. These works primarily focus on individual objects, whereas scaling to room-sized environments requires the robot to efficiently and effectively explore the large-scale 3D space for meaningful interactions. 

We introduce \textbf{Ditto in Real World}, a full-fledged pipeline for the mobile manipulator to build the articulation model of an unfamiliar environment through self-directed exploration. Based on the static models acquired from SLAM or other 3D reconstruction techniques, the robot discovers and physically interacts with articulated objects in the environment. After that, the robot captures the change in the object's state before and after the interaction and infers the articulation properties. 

The foremost challenge is determining the ... (base reposition?)
\todo{}


Figure~\ref{fig: teaser} illustrates the high-level steps of our approach...
\todo{}

To our knowledge, this work is the first to introduce a fully autonomous exploration and reconstruction pipeline for articulation objects on a room-level scale. The empirical evaluation shows that the reconstructed articulation models significantly improve performance in mobile manipulation tasks. More importantly, these models enhance the robot's ability for long-horizon planning in complex indoor environments.

==> backup/_approach.tex <==

% The movement of articulated parts is restricted by articulation constraints. Ensuring that the force applied to the object adheres to kinematic constraints is crucial during interaction. Nevertheless, the articulation constraints remain unknown during the exploration phase. 


To interact, ...

To reposition, ...
% Moreover, the articulation constraints remain unknown before the manipulation. Articulation constraints play a pivotal role in determining whether the motion trajectories fall within the arm's working space. The inability to accurately parameterize the action sequence hinders the robot's capability to adapt its base position for subsequent manipulation and often results in failures like self-collision or limited joint configuration. To overcome these challenges, we propose a straightforward strategy for repositioning the base during manipulation trials.


The movement of articulated parts is restricted by articulation constraints. Ensuring that the force applied to the object adheres to kinematic constraints is crucial during interaction. Nevertheless, the articulation constraints remain unknown during the exploration phase. Alternatively, we use geometric priors to estimate the articulation flow at the current grasp location.  In our approach, we estimate the surface normals of the point cloud observation from the wrist camera at each time step. These surface normal estimates predict how the object part would move under articulated motion without relying on the articulation model. To prevent potential damage to hardware or furniture, we incorporate admittance control, introducing slight compliance to kinematic constraints.

Moreover, the articulation constraints remain unknown before the manipulation. Articulation constraints play a pivotal role in determining whether the motion trajectories fall within the arm's working space. The inability to accurately parameterize the action sequence hinders the robot's capability to adapt its base position for subsequent manipulation and often results in failures like self-collision or limited joint configuration. To overcome these challenges, we propose a straightforward strategy for repositioning the base during manipulation trials.



In our practical experience, manipulation often faces challenges like self-collision and joint limitations. Upon detecting a failure, the robot repositions itself and makes another attempt at manipulating the object to avoid potential damage.





In our practice, we estimate the surface normals of the point cloud observation from the wrist camera at each time step. The surface normal estimates how the object part would move under articulated motion without needing the articulation model. To prevent potential damage to hardware or furniture, we implement admittance control, which imparts slight compliance to the kinematic constraints. In our experience, the manipulation often encounters challenges such as self-collision and joint limitations. When a failure is detected, the robot will reposition itself and make another attempt at manipulating the object. 

subject to
the articulation constraints

Articulated objects are constrained by the 
To make sure the force applied to object is comply with the kinematic constraint. 
as we don't have the articulation model, We estimate the articulation flow at the current grasp location by geometry priors.

In our practice, we use normal estimation to estimate the surface normals of the point cloud observation from arm wrist camera.

To prevent potential damage to hardware or furniture, we implement admittance control, which imparts slight compliance to the kinematic constraints. In our experience, the manipulation often encounters challenges such as self-collision and joint limitations. When a failure is detected, the robot will reposition itself and make another attempt at manipulating the object. 

however, base reposition still is problem


\noindent \textbf{Heuristic Interaction.}
In the exploration, the goal is to interact with the object and collect articulation observations, so that we can build the scene-level articulation model based on these observations. Nevertheless, interacting with the object without an articulation model poses challenges. 
% pull direction
XX
% base reposition
During the interaction, the robot needs to infer the motion trajectory of the mobile part of the object. Along with this trajectory, the robot can adjust its base position and ensure the following manipulation is within its working space. This can avoid the failures such as self-collision or reaching joint limits. The challenge is the motion trajectory depends on the underlying kinematic constraints of the object, which is only available when the articulation model is known.


\noindent \textbf{Base Reposition.}


The crucial insight is that even if the manipulation attempt fails, it can provide crucial information about the joint type. For joint classification, we utilize plane detection on the wrist camera that can track the pose changes of the object's mobile part. Depending on the presence of rotation, we classify the joint as either revolute or prismatic. If rotation is detected, whether clockwise or counterclockwise, we further distinguish the rotation direction as left or right revolute. While the joint type cannot substitute the need for a complete articulation model, this information can be leveraged to adjust the base for collecting better motion observations. we developed heuristic strategies for base repositioning in the exploration stage. For revolute joints, the robot moves to the same side as the rotation to preserve more space for subsequent manipulation. In the case of prismatic joints, the robot moves away from the object to allocate more space for the translation movements. Considering the reaching limit of the arm, the new base position is set within a fixed distance,~\ie, 30 cm, away from the interaction hotspot. It's important to note that these strategies do not account for object size and position, resulting in sub-optimal manipulation results. Nonetheless, they play a crucial role in the articulation model-building process by providing motion signals beyond static observations.

==> backup/_approach_2.tex <==



To avoid self-collision or reaching joint limits, we randomly sample a set of base positions within a certain range of the object. Among these base positions, we select the position that can reach the most poses on the trajectory as our final base position during execution. In task-level planning settings that involves manipulating multiple object and object-to-object collision might occur. We first extract the bounding box of the mobile part based on the mobile part segmentation of the predicted articulation model. By sampling  different joint configurations, we then compute the transformation of the mobile part along the articulation trajectory based on articulation parameters. If the box of different object is overlapped or fall within certain distance threshold, we detect the collision. We keep sampling until find a set of configuration that won't cause collision. After that we compute the articulation trajectories based on the result configuration for each object. The robot then execute the trajectory based on the sampled trajectory.





For single object manipulation, we randomly sample a set of base positions within a certain range of the object. Among these base positions, we select the position that can reach the most poses on the trajectory as our final base position during execution. This allow us to to avoid self-collision or reaching joint limitation



Given the inferred articulation and grasp point $p$, we can analytically compute a multi-step action trajectory as demonstrated in Section~\ref{sec: preliminary}. Unlike in the exploration stage, we now have the full trajectory and no longer need to re-compute each step when actuating the articulated part. To avoid self-collision or reaching joint limitation due to sub-optimal base position, we propose to use the action trajectory for arm and base planning before action.

For single object manipulation, we randomly sample a set of base positions within a certain range of the object. Among these base positions, we select the position that can reach the most poses on the trajectory as our final base position during execution.
%
For task-level planning, we first extract the bounding box of the mobile part based on the mobile part segmentation of the predicted articulation model.
Given the joint configuration, we then compute the transformation of the mobile part along the articulation trajectory based on articulation parameters. If the box of different object is overlapped or fall within certain distance threshold, we detect the collision. By randomly sample different configuration of each object, we can find a set of configuration that won't cause collision. After that we compute the articulation trajectories based on the result configuration for each object. The robot then execute the trajectory based on the sampled trajectory. This prevent the self-collisions and obejct-to-obejct collision

% For each object, we first find the interaction hotspot (see~\todo{section}). Based on the articulation model and interaction hotspot,  we can evenly sample $n$ grasp points along the articulation trajectory. These grasp points represent the poses of the end effector when following the trajectory. Base on these poses, we randomly sample a set of base positions close to the object. Among these base positions, we select the position that can reach the most end effector pose as our final base position during execution.
 




Oppose to the heuristic exploration, the inferred articulation model give us analytically compute a multi-step articulation trajectory without the need
to stop and re-compute each step to actuate the articulated part. To complete avoid self collision or joint limitation due to sub-optimal base position, we propose to use the multi-step articulation trajectory for arm and base planning. 

For each object, we first find the interaction hotspot (see~\todo{section}). Based on the articulation model and interaction hotspot,  we can evenly sample $n$ grasp points along the articulation trajectory. These grasp points represent the poses of the end effector when following the trajectory. Base on these poses, we randomly sample a set of base positions close to the object. Among these base positions, we select the position that can reach the most end effector pose as our final base position during execution.
 
~\todo{figure}
For task-level planning, we first extract the bounding box of the mobile part based on mobile part segmentation of predicted articulation model.
Given the joint configuration, we then compute the transformation of the mobile part along the articulation trajectory based on articulation parameters. If the box of different object is overlapped or fall within certain distance threshold, we detect the collision. By randomly sample different configuration of each object, we can find a set of configuration that won't cause collision. After that we compute the articulation trajectories based on the result configuration for each object. The robot then execute the trajectory based on the sampled trajectory. This prevent the self-collisions and obejct-to-obejct collision




\noindent \textbf{Online planning.}
why? solve self-collision and joint limitations.

After registration
we have joint axis (seg?)
compute action trajectories (cite FlowBot3D)
sample n poses along the trajectoris

sample base pose within a certain area
find the most feasible plan for manipulation

For LH planning, ...











% Finally, the network outputs the articulation joint parameters, joint state, and part segmentation of each articulated object. To build the final articulation models, we aggregate the estimated object-level articulation models into a scene-level model.


% In previous interactions, the robot collects egocentric observations of the object before and after the interactions. Based on these observations, we can observe changes in the articulated configurations of the object. Based on these changes, we use an articulation network to infer the articulation model. The network is built on top of prior work DiTH~\cite{hsu2023ditto}. 

% For each interaction pair, the robot captures the observation point clouds $P$ and $P'$ by grasping the interaction hotspots $c$ and $c'$. To incorporate the knowledge of the interaction, we use the contact regions of the interaction as part of the input to our network. We create Gaussian heatmaps centered around the $c$ and $c'$ over the point cloud $P$ and $P'$, respectively. These heat maps represent the regions where interactions occur. The locations of contact regions during interaction reveal a vital clue about the mobile part region and the underlying kinematic constraint. Therefore, we feed both the point cloud observations and the heatmaps of contact regions into the network for articulation inference. Finally, the model simultaneously predicts the 3D geometry and articulation model of the object.


% Given a pair of visual observations of an object before and after its articulated motion, the model simultaneously predicts the 3D geometry and articulation model of the object. Our agent physically interacts with the object and then collects the observations. So we incorporate the knowledge of the interaction and use the contact regions of the interaction as part of the input to our network.



% After each successful interaction, we observe changes in the expressed 

% After each effective interaction, we observe changes in the articulated configurations of the object. The robot collects egocentric observations of the object before and after the interactions. We use an articulation network to infer the articulation model from these observations.

% The network is built on top of prior work DiTH~\cite{hsu2023ditto}. Given a pair of visual observations of an object before and after its articulated motion, the model simultaneously predicts the 3D geometry and articulation model of the object. Our agent physically interacts with the object and then collects the observations. So we incorporate the knowledge of the interaction and use the contact regions of the interaction as part of the input to our network.

% For each interaction pair, the robot captures the observation point clouds $P$ and $P'$ by interacting at the corresponding contact locations $c$ and $c'$. We create Gaussian heatmaps centered around the $c$ and $c'$ over the point cloud $P$ and $P'$, respectively. These heat maps represent the regions where interactions occur. The locations of contact regions during interaction reveal a vital clue about the mobile part region and the underlying kinematic constraint. Therefore, we feed both the point cloud observations and the heatmaps of contact regions into the network for articulation inference.

% Finally, the network outputs the articulation joint parameters, joint state, and part segmentation of each articulated object. To build the final articulation models, we aggregate the estimated object-level articulation models into a scene-level model.


==> backup/_approach_3.tex <==
\section{Approach}
In this section, we elaborate on the details of the hardware as well as our full-stack approach, including physical exploration, articulation inference, and articulation planning. This enables our robot to build the scene-level articulation model and perform long-horizon tasks that involve manipulating articulated objects.


\subsection{Hardware}
Our mobile manipulator robot is equipped with a four-wheeled omnidirectional base and a Kinova Gen 3 7DoF arm. We use an Intel NUC computer to process all communication among components, including sensors, the base, and the arm. The robot utilizes a forward-facing Kinect camera to capture RGBD images as ego-centric observations. Another Intel Realsense RGBD camera is mounted on the wrist of the arm to provide detailed observations during manipulation. Additionally, the robot employs an affordable short-range laser rangefinder, the Hokuyo URG-04lx, for mapping and localization purposes. The arm is equipped with a 3D-printed soft robotic gripper. The soft robotic gripper offers flexibility and compliance during articulation manipulation, minimizing the risk of damage to hardware or furniture. 


\subsection{Physical Exploration}
\noindent \textbf{Interaction Hotspots Discovery.}
In the initial phase, our focus is on identifying potential interaction regions and recognizing articulated objects. We aim to highlight the noteworthy candidate on the map, paving the way for further exploration. Since most objects are designed for human use, it's reasonable to assume that many incorporate components or parts intended for human-hand interaction. We particularly observe that handle designs are prevalent in everyday environments such as kitchens. Consequently, we simplify the problem by focusing on handle detection. 

For handle detection, we use a YOLO detector~\cite{redmon2016you} trained on the DoorDetect dataset~\cite{Arduengo_2021}. Given an image, the detector outputs the bounding box of the detected handle. Based on the localization of the robot, the detection can be converted into the map frame, so that the robot can revisit the location in the further stage. We then use non-maximum suppression to remove duplicate handle detection on the same object.

Upon identifying the candidate of interest on the map, the robot can navigate directly to the object. However, due to the limited precision of the localization module, the handle location can only offer a general indication of the object's position, lacking the precision required for articulation manipulation. Based on the robot's current egocentric observation, we use the handle detector to retrieve the bounding box of the handles. Subsequently, the center point of the bounding box is selected as the interaction hotspot. This location is then converted into the end effector frame by leveraging depth sensor information. The robot proceeds to grasp the interaction hotspot to start interacting with the object. 

\noindent \textbf{Exploratory Interaction}
% two challenges - interaction and repositioning
Interacting with the object during the exploration phase is challenging due to the lack of prior knowledge about the articulated object. While the movement of articulated parts is restricted by articulation constraints, the articulation constraints remain unknown during the exploration phase. Articulation constraints play a pivotal role in determining whether the motion trajectories fall within the arm's working space. The inability to accurately parameterize the action sequence hinders the robot's capability to adapt its base position for subsequent manipulation and often results in failures like self-collision or limited joint configuration. To overcome these challenges, we propose a heuristic strategy to avoid the limitations.

% solution for interaction
To ensure that the applied force on the object complies with kinematic constraints, we utilize geometric priors to infer the next action at the current grasp location. In our approach, we estimate the surface normals of the point cloud observation from the wrist camera at each time step. These surface normal estimates predict how the object part would move under articulated motion without relying on the articulation model. To prevent potential damage to hardware or furniture, we incorporate admittance control, introducing slight compliance to kinematic constraints.

% solution for base repositioning
% \noindent \textbf{Base Reposition.}
Without the long-term action trajectory, the robot often results in a sub-optimal base position and often faces challenges like self-collision and joint limitations. To overcome the challenge, upon detecting a failure, the robot repositions itself and makes another attempt at manipulating the object. One insight is that even if the manipulation attempt fails, it can provide crucial information about the joint type. For joint classification, we utilize plane detection on the wrist camera that can track the pose changes of the object's mobile part. Depending on the presence of rotation, we classify the joint as either revolute or prismatic. If rotation is detected, whether clockwise or counterclockwise, we further distinguish the rotation direction as left or right revolute. While the joint type cannot substitute the need for a complete articulation model, this information can be leveraged to adjust the base for collecting better motion observations. we developed heuristic strategies for base repositioning in the exploration stage. For revolute joints, the robot moves to the same side as the rotation to preserve more space for subsequent manipulation. In the case of prismatic joints, the robot moves away from the object to allocate more space for the translation movements. Considering the reaching limit of the arm, the new base position is set within a fixed distance,~\ie, 30 cm, away from the interaction hotspot. It's important to note that these strategies do not account for object size and position, resulting in sub-optimal manipulation results. Nonetheless, they play a crucial role in the articulation model-building process by providing motion signals beyond static observations.

\noindent \textbf{Motion Observation Collection.}
The inference of the articulation model heavily depends on visual observations collected during interactions. However, visual occlusion poses a significant challenge in mobile manipulation, especially when the camera is often obstructed by the robot arm or object parts during the manipulation of articulated objects. To enhance the accuracy of the estimated articulation model, observations must capture substantial articulation motions and provide a complete view of the object's interior.

To tackle this issue, we collect observations only before and after interactions, minimizing occlusion during the interaction itself. This collection approach enables the robot to adjust its position without being constrained by arm configuration limits. In practice, the robot will move a small fixed distance away from the object. Empirically, we have observed that this improves the observation coverage and results in more accurate articulation estimation.

\subsection{Articulation Inference}
During prior explorations, the robot collects egocentric observations of the object both before and after the interactions. By analyzing these observations, we can detect changes in the articulated configurations of the object. Utilizing these changes as input, we employ an articulation network to infer the articulation model, building upon the prior work DiTH~\cite{hsu2023ditto}.

For each pair of interactions, the robot acquires observation point clouds $P$ and $P'$ by grasping the interaction hotspots $c$ and $c'$. To integrate knowledge from the interaction, we incorporate the contact regions into our network input by creating Gaussian heatmaps centered around $c$ and $c'$ over the point clouds $P$ and $P'$, respectively. These heatmaps represent the contact regions of interaction and offer insights into the mobile part region and underlying kinematic constraints. Both the point cloud observations and the heatmaps of contact regions are fed into the network for articulation inference. The model then outputs the articulation joint parameters and part segmentation of each articulated object. Finally, we aggregate the estimated object-level articulation models into a scene-level model.

\subsection{Articulation Planning}
% two challenges - self-collision (single object) and object-to-object collisions (multi objects)
~\todo{add figure}
Given the inferred articulation and grasp point $p$, we can infer a multi-step action trajectory as demonstrated in Section~\ref{sec: preliminary}. In contrast to the exploration stage, the complete trajectory is now available, eliminating the need to recalculate each step during the actuation of the articulated part. The trajectory indicates the motion of the end effector and the mobile part. With this information, we can pre-compute the robot poses and potential collisions before executing the action.

To prevent self-collision or reaching joint limits, we use a random sampling approach to generate a set of base positions within a specified range around the object. Among these base positions, we choose the one that can reach the most poses on the trajectory as our final base position during execution. In task-level planning scenarios involving the manipulation of multiple objects where object-to-object collisions may occur, we begin by extracting the bounding box of the mobile part using the segmentation of the predicted articulation model. By sampling various joint configurations, we calculate the transformation of the mobile part along the articulation trajectory based on articulation parameters. If the bounding boxes of different objects overlap or fall within a certain distance threshold, we detect a collision. We continue sampling until we find a set of configurations that avoid collisions. Following that, we compute the articulation trajectories based on the resulting configurations for each object. The robot then executes the trajectory based on the sampled path. In practice, we sample 3 different configurations for each object by interpolating from zero to the maximum state\footnote{The maximum state for the revolute joint and prismatic joint is set as 90 degrees and 15cm respectively.}.


\subsection{System Details}

\noindent \textbf{Manipulation under Estimated Articulation Model.}
After inferring the articulation model of the objects, at each interaction, the robot grasps the interaction hotspot $p \in \mathbb{R}^{3}$ and applies sequential actions that comply with the kinematic constraints until reaching the goal angle $g_r$ for revolute joint, or goal translation $g_p$ for prismatic joint. These sequential actions can be represented as trajectories following FlowBot3D~\cite{}. 

For a revolute joint, the action trajectory lies within the circle within a plane perpendicular to the revolute axis $u^r$. Given a rotation angle $\phi$, the rotation matrix can be defined as follows:
\begin{equation}
    \mathbf{R}(\phi) = \mathbf{I} + \sin \phi [u^r]_\times + (1-\cos\phi) [u^r]_\times^2
    \label{eq:get-rot}
\end{equation}
where $\mathbf{I}$ is identity matrix and $[u^r]_\times$ is the skew-symmetric matrix of $u^r$.
%
By evenly sampling $K$ steps between $0$ and the goal angle $g_r$, the action trajectory can be defined as follows:
\begin{equation}
    \tau_\text{revolute} =\left\{\mathbf{R}\left(\frac{i}{K}{g_r}\right)(p-q)+q\right\}_{\forall i \in[0, K]}
    \label{revolute-traj}
\end{equation}

For prismatic joints, the $K$-step trajectory is defined as the translation of the grasp point $p$ to the goal translation $g_p$.
\begin{equation}
    \tau_\text{prismatic} = \left\{p + \frac{i}{K}g_p {u^p} \right\}_{ i \in[0, K]}
    \label{prismatic-traj}
\end{equation}

\noindent \textbf{Registration.}
Accurate articulation parameters are essential for effective manipulation. However, upon reaching the object, the robot's pose may differ from that observed during the collection of articulation data, possibly due to the precision limit of the localization module. To facilitate planning based on the estimated articulation model, a critical step involves aligning the current observation with the articulation observation. This alignment ensures that the estimated articulation and current observation are synchronized within the same coordinate system. To build an energy-efficient system, we opt for colored ICP~\cite{park2017colored}, given its ability to run swiftly on typical consumer-grade CPUs. Colored ICP leverages color as supplementary information to prevent registration errors along the tangent, especially when geometric features lack sufficient constraints for optimization. Our empirical result shows that direct registration is prone to fail due to noisy and incomplete observations. As a remedy, we remove points that are further away from their neighbors compared to the average for the point cloud. 
% The distance threshold is set as~\todo{} in all our experiments. ~\todo{add plane detection?}

\noindent \textbf{Error Detection and Recovery.}
Interaction failures may arise from uncontrollable issues, such as inaccurate or absent depth information or the gripper slipping away during the interaction. To identify and address these errors, we incorporate a straightforward error detection mechanism. By computing the distance between the observed point cloud before and after the interaction, we can determine whether the mobile part has been displaced by setting a certain threshold.
When an error is detected, the robot repositions itself and attempts the interaction again to recover from the failure state.

\noindent \textbf{Mapping and Navigation.}
We use the Nautilus~\cite{nautilus} tool based on the scene scanning for mapping and ENML~\cite{biswas2016episodic} for the localization during all navigation. 

\noindent \textbf{Base Reposition}
To reposition the base, we use the MOSSE object tracker~\cite{bolme2010visual} to track the relative pose in the end-effector frame between the interaction hotspot and the robot from the video stream. We implement a simple PID controller for the base movement to ensure the robot achieves the desired position.

% \noindent \textbf{Depth completion.}


==> backup/_experiment.tex <==
\section{Experiments}

\input{sections/quant_main}
\input{sections/quant_art}


\begin{figure}[t]
    \centering
    % \includegraphics[width=\linewidth]{figs_pdf/XX.pdf}
    \includegraphics[]{figs_pdf/XX.pdf}
    % \vspace{-5mm}
    \caption{
        \textbf{\todo{Typical challenges in rearrangement task.}}
    }
    % \vspace{-2mm}
    \label{fig: XX}
\end{figure}

% \begin{figure}[t]
%     \centering
%     % \includegraphics[width=\linewidth]{figs_pdf/XX.pdf}
%     \includegraphics[]{figs_pdf/XX.pdf}
%     % \vspace{-5mm}
%     \caption{
%         \textbf{\todo{stacked bars}}
%         Ablation: discuss ablation in each component including
%         no "retry" in exploration stage
%         no error detection / recovery
%         no base adjustment / resample
%         adding noise to AE (we're not compare to other AE method because they are too bad)
%     }
%     % \vspace{-2mm}
%     \label{fig: XX}
% \end{figure}

% \begin{figure}[t]
%     \centering
%     % \includegraphics[width=\linewidth]{figs_pdf/XX.pdf}
%     \includegraphics[]{figs_pdf/XX.pdf}
%     % \vspace{-5mm}
%     \caption{
%         \textbf{\todo{cash flow diagram / stacked bars}}
%         repeatability: Discuss types of error running "exploration" for 20 times
%         repeatability: Discuss types of error running "exploitation" for 20 times
%         nav/relocal failed
%         handle detec failed
%         ae registration failed
%         bad depth
%     }
%     % \vspace{-2mm}
%     \label{fig: XX}
% \end{figure}

\begin{figure}[t]
    \centering
    % \includegraphics[width=\linewidth]{figs_pdf/XX.pdf}
    \includegraphics[]{figs_pdf/XX.pdf}
    % \vspace{-5mm}
    \caption{
        \textbf{\todo{failure modes}}
         single object: self-collision / base position or orientation
         multiple objects: object-object collision/view occlusion    
    }
    % \vspace{-2mm}
    \label{fig: XX}
\end{figure}


\begin{itemize}
    \item \textit{Discussion:} How much does our method fall behind the perfect setting?
    \item \textit{Result:} articulation estimation
    \item \textit{Metrics:} exploration coverage / articulation parameter error
    \item \textit{Baselines:}
    \begin{itemize}
        \item Perfect Camera Setting vs. Onboard Robot Camera
        \item Human Interaction vs. Robot's Self-Directed Interaction
    \end{itemize}
\end{itemize}


\subsection{Experimental Setup}

\noindent \textbf{Scenes.}

\subsection{Evaluation Metrics}

\noindent  \textbf{Articulation Model.}

\noindent  \textbf{Manipulation.}


\subsection{Baselines}
% manipulation
\noindent \textbf{Oracle.}
Perfect camera view and interaction (?).

\noindent \textbf{Heuristic.}
Our exploration stage.

\noindent \textbf{Ours.}
Ditto-based planning.

% articulation estimation
\noindent \textbf{OPDMulti~\cite{}.}
Single RGB

\noindent \textbf{ANCSH~\cite{}.}
Single RGBD

\noindent \textbf{ScrewNet~\cite{}.}
Sequential depth

\noindent \textbf{~\cite{}.}
Sequential rgb

\noindent \textbf{Proprioception Only.}

\subsection{Experimental Analysis}

\noindent \textbf{Self-exploration.}
\begin{itemize}
    \item \textit{Discussion:} How much does our method fall behind the perfect setting?
    \item \textit{Result:} articulation estimation
    \item \textit{Metrics:} exploration coverage / articulation parameter error
    \item \textit{Baselines:}
    \begin{itemize}
        \item Perfect Camera Setting vs. Onboard Robot Camera
        \item Human Interaction vs. Robot's Self-Directed Interaction
    \end{itemize}
\end{itemize}

\noindent \textbf{Articulation Estimation.}
\begin{itemize}
    \item \textit{Discussion:} The drawback of the current approach in MoMa settings.
    \item \textit{Result:} articulation estimation
    \item \textit{Metrics:} articulation parameter error
    \item \textit{Baselines:}
    \begin{itemize}
        \item All AE baselines
    \end{itemize}
\end{itemize}
    
\noindent \textbf{Articulated Object Manipulation.}
\begin{itemize}
    \item \textit{Discussion:} How does the built map help in manipulation?
    \item \textit{Discussion:} Limitation of Heuristic: base planning and long-horizon task planning
    \item \textit{Result:} base planning + arm trajectories (Single object)
    \item \textit{Result:} long-horizon task planning
    \item \textit{Metrics:} Success Rate / Speed
    \item \textit{Baselines:}
    \begin{itemize}
        \item Heuristic vs. Ours
    \end{itemize}
\end{itemize}

\subsection{Limitations}

\noindent \textbf{Environmental Assumption.}
\begin{itemize}
    \item assume plane normal and handle orientation
    \item assume handle exists and is graspable, e.g., dishwasher
\end{itemize}

\noindent \textbf{Hardware or System Design.}
\begin{itemize}
    \item handle too low/high
    \item lidar occlusion / high precision map (environment changes)
    \item exploration stage: large object like fridge
    \item error detection and recovery: when to stop - avoid damaging hardware / stop early when slipping away / rely on plane normals
\end{itemize}

\noindent \textbf{Perception.}
\begin{itemize}
    \item reflective surface
    \item handle detector, e.g., in fridge
\end{itemize}

\noindent \textbf{Error Detection and Recovery.}

==> backup/_formulation.tex <==

to translate the contact point $p$ by a goal translation distance $l_g$:


To obtain a trajectory, we interpolate $K$ angles between 0 and a goal angle $g_r$, and the smooth, $K$-step trajectory\footnote{In practice, the goal translation distance and goal angle is set large enough so that the termination condition (part being fully open) of the policy can be triggered.} that rotates the contact point $p$ by angle $g_r$ about the estimated axis parameterized by $\hat{\boldsymbol{\omega}}$ and $\hat{v}$  is calculated via:

For \textit{prismatic objects}, since the motion direction and the axis direction should be the same, we  just use the normalized flow prediction $f_p$ to compute the prismatic 
 %actuate the object until a stopping condition is reached.  %Qualitative results in \cite{eisner2022flowbot3d} show that the flow vectors prediction quality of prismatic objects is higher than that of revolute objects. 
 %We then normalize the mean learned flow direction as the estimated 
 articulation axis, and we use the estimated axis to compute a smooth, $K$-step trajectory indexed by $i$ to translate the contact point $p$ by a goal translation distance $l_g$:
\begin{equation}
    \tau_\text{prismatic} = \left\{p + \frac{i}{K}l_g {u^p} \right\}_{ i \in[0, K]}
    \label{prismatic-traj}
\end{equation}







These predictions of $\hat{v}$ are visualized as the blue points in the bottom output branch of Fig. \ref{fig:system}. Using the inferred axis direction $\hat{\boldsymbol{\omega}}$ and origin $\hat{v}$, we can interpolate a smooth trajectory: given a contact point $p$, the proposed trajectory should lie on a circle in a plane  perpendicular to the inferred axis parameterized by the normalized direction $\hat{\boldsymbol{\omega}}$ and the origin $\hat{v}$. Formally, with Rodrigues' Formula of Lie algebra, given an angle of rotation $\phi$  about the normalized vector $\hat{\boldsymbol{\omega}}$ we are able to define a rotation matrix as follows:
\begin{equation}
    \mathbf{R}(\phi) = \mathbf{I} + \sin \phi [\hat{\boldsymbol{\omega}}]_\times + (1-\cos\phi) [\hat{\boldsymbol{\omega}}]_\times^2
    \label{eq:get-rot}
\end{equation}

where $\mathbf{I}$ is identity matrix and $[\hat{\boldsymbol{\omega}}]_\times$ is the skew-symmetric matrix of $\hat{\boldsymbol{\omega}}$, and the rotated point $p$ about this inferred axis by angle $\phi$ is given by:
$p' = \mathbf{R}(\phi)(p-\hat{v}) + \hat{v}$.

To obtain a trajectory, we interpolate $K$ angles between 0 and a goal angle $\phi_g$, and the smooth, $K$-step trajectory\footnote{In practice, the goal translation distance and goal angle is set large enough so that the termination condition (part being fully open) of the policy can be triggered.} that rotates the contact point $p$ by angle $\phi_g$ about the estimated axis parameterized by $\hat{\boldsymbol{\omega}}$ and $\hat{v}$  is calculated via:
\begin{equation}
    \tau_\text{revolute} =\left\{\mathbf{R}\left(\frac{i}{K}\phi_g\right)(p-\hat{v})+\hat{v}\right\}_{\forall i \in[0, K]}
    \label{revolute-traj}
\end{equation}


For \textit{prismatic objects}, since the motion direction and the axis direction should be the same, we  just use the normalized flow prediction $f_p$ to compute the prismatic 
 %actuate the object until a stopping condition is reached.  %Qualitative results in \cite{eisner2022flowbot3d} show that the flow vectors prediction quality of prismatic objects is higher than that of revolute objects. 
 %We then normalize the mean learned flow direction as the estimated 
 articulation axis, and we use the estimated axis to compute a smooth, $K$-step trajectory indexed by $i$ to translate the contact point $p$ by a goal translation distance $l_g$:
\begin{equation}
    % \hat{\boldsymbol{\omega}} = \mathrm{Normalize}\left(\sum_{i=1}^N\frac{\mathbf{f}}{||\mathbf{f}||}\right)
    \hat{\boldsymbol{\omega}} = \frac{f_p}{||f_p||},\;\;\tau_\text{prismatic} = \left\{p + \frac{i}{K}l_g\hat{\boldsymbol{\omega}}\right\}_{ i \in[0, K]}
    \label{prismatic-traj}
\end{equation}




Based on the articulation parameters, we can 

applies forces to the object hotspot to produce potential articulated motions.


We explore the problem of building an articulation model of an indoor scene populated with articulated objects. An articulated object consists of multiple parts, and their connecting joints constrain the relative motion between each pair of parts. We assume there exists an initial point cloud observation $P_s \in \mathbb{R}^{N_s \times 6}$ of the scene, where each point is a vector of its $(x, y, z)$ coordinate and $(R, G, B)$ color. $N_s$ is the number of points. This work aims to segment the parts and estimate the articulation models $M$ of the scene through interactive perception. Our approach actively interacts with the objects to estimate their articulation models.

For each object part, we identify the interaction hotspots~\cite{nagarajan2019grounded}, \textit{i.e.}, the locations where the robot can successfully manipulate the articulated objects, and infer the articulation model. The articulation model represents the kinematic constraints between object parts. We parametrize articulation following ANCSH~\cite{li2020category}. Prismatic joint parameters are the direction of the translation axis $u^p \in \mathbb{R}^{3}$ and the joint state $s^p \in \mathbb{R}$. Revolute joint parameters are the direction of the revolute axis $u^r \in \mathbb{R}^{3}$, a pivot point $q \in \mathbb{R}^{3}$ on the revolute axis, and the joint state $s^r \in \mathbb{R}$. The joint state $s^p$ and $s^r$ are the relative changes of the joint state before and after the interaction. 

The process starts with finding interaction hotspots $H_s \in \mathbb{R}^{N_h \times 3}$ from an initial scene observation $P_s$, where $N_h$ denotes the number of interaction hotspots in the scene. From the point cloud observation $P_s$, an affordance prediction model predicts an affordance map $A_s \in \mathbb{R}^{N_s}$ and samples its peak locations as interaction hotspots. 

At each interaction, the robot applies forces to the object hotspot to produce potential articulated motions. The robot captures two egocentric partial point clouds $P \in \mathbb{R}^{N_o \times 3}$ and $P' \in \mathbb{R}^{N_o' \times 3}$ that center on the interaction hotspot before and after the interaction, where $N_o$ and $N_o'$ denotes the number of points on object point clouds. The robot also records the corresponding contact locations $c, c' \in \mathbb{R}^{3}$. Given these object point clouds $P, P'$ and contact locations $c, c'$, an articulation inference model segments the point cloud into static and mobile parts and estimates a set of articulation parameters,~\ie, $\{u^p, s^p\}$ (prismatic) or $\{u^r, q, s^r\}$ (revolute), of the joints connecting two object parts. Finally, we map the estimated articulation model of each object from the global frame. The set of these articulation models constitutes the scene-level articulation model $M$.


==> backup/_intro.tex <==
\section{Introduction}

\begin{comment}
- We want to deploy domestic service mobile robots...
- Limitations of zero-shot approaches 
- Hence we are interested in building an articulated 3D map of the world
- We are thus interested in addressing the ``robot unboxing problem'', where a domestic service mobile robot is introduced to a new home, and it needs to build a model sufficient for it to perform complex tasks accurately and robustly.
- This requires not only manipulating individual objects but also TAMP...
- As such, we need scene-level articulation models...
- Sub-tasks of this problem have been investigated before, including... but we are interested in understanding 1. how to combine all of them to enable a robot to autonomously [do it all], and 2. the performance of SOTA sub-problem approaches at addressing this problem. The overall problem has been investigated in simulation [cite], but 1) without a robot, and 2) without first-person perception limitations.
- We thus contribute:
  1. [Overall system]
  2. [Empirical evaluation of sub-problems and how they integrate into the overall problem]
  3. Empirical results showing that our system [works] and that the resulting articulated 3D map is useful for performing interesting domestic tasks
\end{comment}

% tamp
% unbox problem
% not a single research problem
% system problem - some have been investigated


% Why do we need AE models
Interacting with articulation objects is crucial for the robot to operate in everyday environments. Recent advances in structure sensors and SLAM algorithms~\cite{newcombe2011kinectfusion,newcombe2015dynamicfusion,geiger2011stereoscan} have offered ways to build a map of the environment. These maps facilitate mobile robots to localize themselves, navigate around, and plan for the next actions. Nevertheless, real-world manipulation would require a robot to depart from reconstructing a static scene to unraveling the physical properties of objects. To physically interact with articulation objects, such as cabinets and doors, the robot needs to understand their kinematics and articulation properties. From a task planning perspective, static 3D models cannot fully represent real-world situations where regions can be partially occupied, doors can be half open, and multiple doors need to be opened to enable reachability. Similar to how mapping guides navigation, the articulation model allows the robot to plan its actions for object manipulation. Motivated by this goal, this work aims to enable robots to automatically build articulated models of indoor scenes from their purposeful interactions. These models enable zero-shot articulation planners and long-term repeatable interaction with articulation objects.

% How does existing work do with or without AE models?
% with AE: static / category-dependent (/ IP)
% without AE: exploration based
Interacting with articulation objects has been a long-standing challenge in robotics. Previous work has proposed to learn the articulation parameters to enable robotic systems to successfully perform sophisticated planning and control over 3D articulated objects. A series of data-driven approaches have attempted to infer articulation from static visual observations by training models on large 3D datasets~\cite{li2020category,weng2021captra}. These models rely on category-level priors and suffer from appearance ambiguity, limiting their generalizations to a handful of preset categories. Another line of research uses online perception~\cite{} to infer a sequential interaction policy that reveals the object’s hidden part geometry and kinematics. These works primarily focus on individual objects, whereas scaling to room-sized environments requires the robot to efficiently and effectively explore the large-scale 3D space for meaningful interactions. Without the explicit modeling of articulation, these methods cannot either do long-horizon planning or guarantee long-term repeatable interactions given different base positions or view angles. The closest work~\cite{hsu2023ditto} aims to build the articulation model of an indoor environment through a robot’s self-directed exploration, yet it focuses solely on building digital twins without real-world evaluation. Plus, it simplifies the physical exploration in simulation and is not directly transferable in real mobile manipulators. 

% How do existing work get AE models? Why is it not enough for scene-level challenges?
% Understanding object articulation has been a long-standing challenge in computer vision and robotics. In recent years, a series of data-driven approaches have attempted to infer articulation from static visual observations by training models on large 3D datasets~\cite{li2020category,weng2021captra}. These models rely on category-level priors, limiting their generalizations to a handful of preset categories. Category-agnostic approach~\cite{} uses the single image of the object in its initial state, suffering from the ambiguity of articulation despite the similar object appearance. Another line of research~\cite{hausman2015active,martin2014online} uses interactive perception~\cite{bohg2017interactive}. They leverage physical interaction to emit visual observations of articulated motions from which they estimate the articulation properties. These works primarily focus on individual objects, whereas scaling to room-sized environments requires the robot to efficiently and effectively explore the large-scale 3D space for meaningful interactions. 

We introduce \textbf{Ditto in Real World}, a full-fledged pipeline for the mobile manipulator to build the articulation model of an unfamiliar environment through self-directed exploration. Based on the static models acquired from SLAM or other 3D reconstruction techniques, the robot discovers and physically interacts with articulated objects in the environment. After that, the robot captures the change in the object's state before and after the interaction and infers the articulation properties. 

The foremost challenge is determining the ... (base reposition?)
\todo{}


Figure~\ref{fig: teaser} illustrates the high-level steps of our approach...
\todo{}

To our knowledge, this work is the first to introduce a fully autonomous exploration and reconstruction pipeline for articulation objects on a room-level scale. The empirical evaluation shows that the reconstructed articulation models significantly improve performance in mobile manipulation tasks. More importantly, these models enhance the robot's ability for long-horizon planning in complex indoor environments.

==> sections/acknowledgments.tex <==

\section*{Acknowledgments}
Thanks XX for paper review
Thanks Gu-Cheol Jeong and Dongmyeong Lee for helps in 3D printed component

==> sections/quant_lh.tex <==
\begin{table}[t]
    \scriptsize
    \centering
    \vspace{3mm}
    \caption{Results of Scene-level Manipulation}
    % \vspace{3mm}
    \resizebox{\columnwidth}{!}{%
    \begin{tabular}{l|c|cc}
    \toprule
\raisebox{\dimexpr-1\normalbaselineskip-2\cmidrulewidth-2\aboverulesep}[0pt][0pt]{Method} & \multicolumn{1}{c|}{Long-horizon Manipulation} & \multicolumn{2}{c}{Failure Modes} \\
      \cmidrule{2-4}
      & Success Rate\,$\uparrow$ & {\shortstack[c]{Collision\,$\downarrow$}} & {\shortstack[c]{Occlusion\,$\downarrow$}} \\
     \midrule
     Random & 0.23 & 0.50 & 0.27 \\
     Ours & 0.73 & 0.27 & 0.00 \\
     \bottomrule
    \end{tabular}
    }
    \label{tab: long_horizon}
    \vspace{-5mm}
\end{table}
